Time-Critical Influence Maximization in Social Networks with Time-Delayed Diffusion Process

Influence maximization is a problem of finding a small set of highly influential users, also known as seeds, in a social network such that the spread of influence under certain propagation models is maximized. In this paper, we consider time-critical influence maximization, in which one wants to maximize influence spread within a given deadline. Since timing is considered in the optimization, we also extend the Independent Cascade (IC) model and the Linear Threshold (LT) model to incorporate the time delay aspect of influence diffusion among individuals in social networks. We show that time-critical influence maximization under the time-delayed IC and LT models maintains desired properties such as submodularity, which allows a greedy approximation algorithm to achieve an approximation ratio of $1-1/e$. To overcome the inefficiency of the greedy algorithm, we design two heuristic algorithms: the first one is based on a dynamic programming procedure that computes exact influence in tree structures and directed acyclic subgraphs, while the second one converts the problem to one in the original models and then applies existing fast heuristic algorithms to it. Our simulation results demonstrate that our algorithms achieve the same level of influence spread as the greedy algorithm while running a few orders of magnitude faster, and they also outperform existing fast heuristics that disregard the deadline constraint and delays in diffusion.

==> general.tex <==
\note{luwei: Old version from December 2011.  To be cleaned up soon.}

Extending the result of IC-DM and LT-DM to the general threshold model proposed in~\cite{kempe03}.
An idea is to make threshold function $f_v(\cdot)$ to take multisets, allowing multiple activation attempts of $u$ on $v$, one per meeting after $u$ has been activated.

\paragraph{Multiple Chances of Activation Attempts}
In the IC-DM model, suppose $u$ is now allowed to attempt to activate $v$ once per meeting, as long as $v$ is not already active.
We can also assume that the influence probability $p_{u,v}$ decays as $u$ attempts more, since its pursuasiveness tends to become weaker and weaker.
Actually, the single chance assumption is an extreme case of the decay, because we can view it as $p_{u,v}$ decays abruptly after the very first attempt.

Also, in the LT-DM model, although an effective neighbor $u$ of $v$ would possibly meet multiple times before $v$ becomes active, we just counted $u$'s weight $b_{u,v}$ once.
A similar generalization is to make the weight $b_{u,v}$ decay in subsequent meetings.
We can view it as if a new copy of $u$ were created and meeting $v$, but a subsequent copy's influence weight is smaller than that of precedent copies. 

\textcolor{red}{The question is can we generalize these two models to something similar to Triggering Set, and obtain interesting results from them?
The submodularity should hold; we can prove it on a layered graph constructed based on $G$ and $\tau$.}

